Physics-Informed Neural Operator for Learning Partial Differential Equations

In this paper, we propose physics-informed neural operators (PINO) that combine training data and physics constraints to learn the solution operator of a given family of parametric Partial Differential Equations (PDE). PINO is the first hybrid approach incorporating data and PDE constraints at different resolutions to learn the operator. Specifically, in PINO, we combine coarse-resolution training data with PDE constraints imposed at a higher resolution. The resulting PINO model can accurately approximate the ground-truth solution operator for many popular PDE families and shows no degradation in accuracy even under zero-shot super-resolution, i.e., being able to predict beyond the resolution of training data. PINO uses the Fourier neural operator (FNO) framework that is guaranteed to be a universal approximator for any continuous operator and discretization-convergent in the limit of mesh refinement. By adding PDE constraints to FNO at a higher resolution, we obtain a high-fidelity reconstruction of the ground-truth operator. Moreover, PINO succeeds in settings where no training data is available and only PDE constraints are imposed, while previous approaches, such as the Physics-Informed Neural Network (PINN), fail due to optimization challenges, e.g., in multi-scale dynamic systems such as Kolmogorov flows.

==> macros.tex <==

\newcommand{\A}{A}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\U}{U}
\newcommand{\LL}{\mathsf{L}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cW}{\mathcal{W}}

% F for the Fourier transform
% G for the target operator

\newcommand{\F}{\mathcal{F}}
\renewcommand{\G}{\mathcal{G}}
\newcommand{\Gtrue}{\mathcal{G}^{\dagger}}
% \newcommand{\L}{\mathcal{L}}
\newcommand{\Ldata}{\mathcal{L}_{data}}
\newcommand{\Lpde}{\mathcal{L}_{pde}}
\newcommand{\Lanchor}{\mathcal{L}_{op}}
\newcommand{\Lop}{\mathcal{L}_{op}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\Jdata}{\mathcal{J}_{data}}
\newcommand{\Jpde}{\mathcal{J}_{pde}}

\newcommand{\T}{T}
\newcommand{\Td}{T^{\dagger}}
\newcommand{\Sd}{S^{\dagger}}

\newcommand{\dt}{\mathrm{d}t}

\newcommand{\K}{\mathcal{K}}
\newcommand{\vdown}{\check{v}}
\newcommand{\vup}{\hat{v}}

\theoremstyle{definition}\newtheorem{definition}{Definition}
\theoremstyle{plain}\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{remark}\newtheorem{remark}{Remark}
% \theoremstyle{plain}\newtheorem{thm}{Theorem}
% \theoremstyle{remark}\newtheorem{remark}{Remark}
% \theoremstyle{definition}\newtheorem{defin}{Definition}

%Kamyar's
\newcommand{\OpClass}{\mathcal{H}}
\newcommand{\Comp}{\mathcal{C}}
\newcommand{\constraint}{\textit{Conts}}
\newcommand{\Loss}{\mathcal{L}}
% \newtheorem{proof}{Proof}[section]
\newtheorem{proof*}{Proof}[section]

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\wb}{\overline}


==> sections/4-_removed_.tex <==
\section{Generalization in Physic Informed Neural Operator}
When a neural operator is trained on a limited set of training data points, it is desirable that it generalizes to new data points. In this section, we establish the generalization properties of operator learning and study how access to both physics constraints and data enhances the sample complexity. ~\cite{devroye2013probabilistic}. 
%
% In many settings, especially in   PDEs, for any given $a$, $u=\Ftrue(u)$ is uniquely specified. This is known as the realizable setting. We first study this setting and then   extend our generalization theory to stochastic outputs, e.g., SDE, where \(a_j,u_j \sim \mu\) are i.i.d. samples drawn from some probability measure \(\mu\) supported on \(\A\times\U\). 
Let \(D,R,D'\), and \(,R'\) denote any sets, and $\A$ and $\U$ measurable classes of functions, from $D\rightarrow R$ and $D'\rightarrow R'$, respectively, with respect to a sigma algebra $\sigma(\A\times\U)$. $\OpClass$ denotes a class of operators from $\A\rightarrow\U$, and $\ell:\F\times\U\rightarrow[0,1]$ a real valued loss function where the $\F$-section of $\ell$ is measurable and integrable with respect to a probability measure \(\mu\) supported on 
\(\A\times\U\). Therefore, the optimal loss $\Loss^*:=\inf_{G\in\OpClass} \E_{a,u \sim \mu}\left[ \ell\left(u ,G(a)\right)\right]$ is well-defined. For any $G\in\OpClass$, let $\Loss(G):= \E_{a,u \sim \mu}\left[ \ell\left(u ,G(a)\right)\right]$ denote the expected loss, and given a dataset of $N$ data pints \(\{a_j, u_j\}_{j=1}^N\) where 
\((a_j,u_j) \sim \mu\), the empirical loss is denoted as $\Loss_N(G):= \frac{1}{N} \sum_{j=1}^N \ell\left(u_j ,\G(a_j)\right)$. 

We aim to find an operator $G$ such that its performance is close to $\Loss^*$. We follow the empirical risk minimization principle (ERM)~\citep{Vapnik1998} , i.e., minimizing $\Loss_N(G)$ over the space of operators $\OpClass$ and provide statistical sample complexity guarantee for a resulting operator. Following the notation of Rademacher complexity in classical supervised learning~\citep{bartlett2002rademacher}, we define the complexity of operator class $\OpClass$ accompanied with the loss function as follows, 
\begin{align}
\Comp_\ell(\OpClass,N):=\E_{a_i,u_i \sim \mu,\xi_i}\left[\sup_{G\in\OpClass}\frac{1}{N}\sum_{i=1}^N\xi_i\ell\left(u_i ,G(a_i)\right)\right] 
\end{align}



\begin{theorem}[Generalization bound]\label{thm:generalizaion}
Given a data set of $N$ data pints \(\{a_j, u_j\}_{j=1}^N\) where 
\((a_j,u_j) \sim \mu\) are i.i.d. samples drawn from some probability measure \(\mu\) supported on 
\(\A\times\U\), for any $\epsilon>0$, and any $\G$
such that,
\begin{equation}
\Loss_N(G)\leq \inf_{G'\in\OpClass} \Loss_N(G')+\epsilon
\end{equation}
we have, 
\begin{align}
\Loss(G) - \Loss^*\leq 4\Comp_\ell(\OpClass,N) + \sqrt{\frac{2\log(1/\delta)}{N}}+2\epsilon
\end{align}
with probability at most $1-\delta$, and $\Comp_\ell(\OpClass,N)$ denotes the complexity of operator class $\OpClass$.
\end{theorem}
Theorem~\ref{thm:generalizaion} states that when $\Comp_\ell(\OpClass,N)$ is $o(1)$, $\Loss(G) \rightarrow \Loss^*$ when $\epsilon\rightarrow0$ and $N\rightarrow\infty$. In many applications of neural operators, e.g., in PDEs, in addition to the dataset, we have physical or mathematical side information, e.g. divergence-free constraint on outputs, gradient information on the boundary, which is the setting of PINO. Given the operator class $\OpClass$, e.g., space of neural operator with $\Theta$ as the space of parameters, imposing a set of constraints, significantly reduces the complexity of the operator class $\Comp_\ell(\OpClass,N)$, resulting in a better generalization bound. For a given set of constraints $\constraint$, and operator $G\in \OpClass_\constraint$ is $G$ satisfies the constraints in $\constraint$. Therefore, the effective complexity is $\Comp_\ell(\OpClass\cap\OpClass_\constraint,N)$ which captures the presence of constraints. For example, when a full specifying PDE equation is given, there is only one operator satisfying PDE equation, therefore, $\Comp_\ell(\OpClass,N)$ is constant resulting in significant improvement in the sample complexity.  


\begin{proof}\label{proof:generalizaion} 
Let $G\in\OpClass$ be an operator such that,
\begin{align}
\Loss_N(G)\leq \inf_{G'\in\OpClass} \Loss_N(G')+\epsilon
\end{align}
and let $\wb G\in\OpClass$ be an operator such that,
\begin{align}
\Loss(\wb G)\leq \Loss^* +\epsilon
\end{align}
Using these definitions, we have,

\begin{align*}
\Loss(G) - \Loss^*&\leq \Loss(G) - \Loss(\wb G) +\epsilon\\
&= \Loss(G) -  \Loss_N(G) + \Loss_N(G) - \Loss(\wb G) +\epsilon\\
&= \Loss(G) -  \Loss_N(G) + \Loss_N(G) -  \Loss_N(\wb G) + \Loss_N(\wb G) - \Loss(\wb G) +\epsilon\\
&\leq \Loss(G) -  \Loss_N(G) + \Loss_N(\wb G) - \Loss(\wb G) +2\epsilon
\end{align*}
Therefore, we have,

\begin{align*}
\Loss(G) - \Loss^*&\leq 2\sup_{G'\in\OpClass}|\Loss(G') -  \Loss_N(G')| +2\epsilon
\end{align*}
Following the argument in the classical theory of Rademacher complexity ~\citep{bartlett2002rademacher,wainwright2019high} (e.g. Theorem 4.10 of \citep{wainwright2019high}), we have, 

\begin{align*}
\sup_{G'\in\OpClass}|\Loss(G') -  \Loss_N(G')| \leq 2\Comp_\ell(\OpClass,N) + \sqrt{\frac{2\log(1/\delta)}{n}}
\end{align*}
Therefore, we have, 

\begin{align*}
\Loss(G) - \Loss^*&\leq 4\Comp_\ell(\OpClass,N) + \sqrt{\frac{2\log(1/\delta)}{n}}+2\epsilon
\end{align*}


\end{proof}




